Absolutely continuous spectrum for the Anderson model on a tree: a geometric proof of Klein's theorem

We give a new proof of a version of Klein's theorem on the existence of absolutely continuous spectrum for the Anderson model on the Bethe Lattice at weak disorder.

==> probac.tex <==
\input rixmax
%\input epsf
\font\text=pplr at 10pt
\font\it=pplri at 10pt
\font\bold=phvb at 10pt
%\draftmode
%\magnification 1100
        \hsize = 5.9 true in
        \hoffset = 0.45 true in
        \baselineskip = 18pt

%\def\mcomment#1{}
\footline={\hfil}
\footline={\hss\tenrm\folio\hss}
\def\half{{{1}\over{2}}}
\def\hd#1{\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000}
\def\HB{\overline\HH}
\def\BB{{\Bbb B}}
\def\cd{{\rm cd}}
\def\dist{{\rm dist}}

\text
\centerline{\bold Absolutely continuous spectrum for the Anderson model on a tree:}
\vskip 10 pt
\centerline{\bold a geometric proof of Klein's theorem}
\vskip 20 pt

\centerline{Richard Froese}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{University of British Columbia}
%\medskip
\centerline{Vancouver, British Columbia, Canada}
\bigskip
\centerline{David Hasler}
\medskip
\centerline{Department of Mathematics}
%\medskip
\centerline{University of Virginia}
%\medskip
\centerline{Charlottesville, Virginia, USA}
\bigskip
\centerline{Wolfgang Spitzer}
\medskip
\centerline{Department of Physics}
%\medskip
\centerline{International University Bremen}
%\medskip
\centerline{Bremen, Germany}
\vskip 20pt
\centerline{\today}

\input statement
\input mu3bdd
\input refs
\rixend


==> refs.tex <==
\vfill\eject
\hd{Acknowledgements}

R.~F.\ would like to thank Rafe Mazzeo for useful conversations.
D.~H.\ and W.~S.\
would like to thank the Department of Mathematics at the University of
British Columbia for hospitality.

\hd{References}
\parindent = 0pt
\tolerance = 1000

[Ai] M.~Aizenman, {\it Localization at weak disorder: some elementary bounds},
Rev.~Math.~Phys., {\bf 6}, 1163--1182, 1994.
\medskip

[AM] M.~Aizenman and S.~Molchanov, {\it Localization at large disorder and at
extreme energies: an elementary derivation}, Commun.~Math.~Phys., {\bf 157},
245--278, 1993.

[ASW] M.~Aizenman, R.~Sims and S.~Warzel, {\it Stability of the Absolutely 
Continuous Spectrum of Random Schr\"odinger Operators on Tree Graphs,}
to appear in Prob.~Theor.~Rel.~Fields, {\tt math-phys/0502006}.

[An] P.W.~Anderson, {\it Absence of diffusion in certain random lattices},
Phys.~Rev., {\bf 109}, 1492--1505, 1958.

[D] S.A.~Denisov, {\it On the preservation of absolutely continuous spectrum 
for Schrodinger operators}, {\tt math-phys/0501046}.

[FHS] R.~Froese, D.~Hasler and W.~Spitzer, {\it Transfer matrices, hyperbolic
geometry and absolutely continuous spectrum for some discrete Schr\"odinger 
operators on graphs}, to appear in J.~Func.~Anal., {\tt mp-arc:04-244}.

[K1] A.~Klein, {\it Extended States in the Anderson Model on the Bethe
Lattice}, Advances in Math., {\bf 133}, 163--184, 1998, {\tt mp-arc:94-236}.

[K2] A.~Klein, {\it Spreading of wave packets in the Anderson model on the 
Bethe lattice}, Commun.~Math.~Phys., {\bf 177}, 755--773, 1996, {\tt mp-arc:95-481}.

[KLS] A.~Laptev, S.~Naboko and O.~Safronov, {\it Absolutely continuous 
spectrum of Schr\"odinger operators with slowly decaying and oscillating 
potentials}, Commun.~Math.~Phys., {\bf  253},  611--631, 2005, {\tt mp-arc:03-383}.

[SS] O.~Safronov and G.~Stolz, {\it Absolutely continuous spectrum of 
Schr\"odinger operators with potentials slowly decaying inside a cone}, 
{\tt mp-arc:05-316}.


==> rixmax.tex <==
\input amssym.def
%\def\Bbb{\bf} %if \Bbb not available
 
%fonts

\font\bold=cmssbx10
\font\smallfont = pplr at 8.5pt
\font\smallit = pplri at 8.5pt
\font\normalfont = pplr at 9.5pt
\font\it = pplri at 9.5pt
\font\marginfont=cmr7

\def\pplfonts{
	\font\tenrm=pplr at 9.5pt
	\font\tensl=pplro at 9.5pt
	\font\eightit=pplri at 8.5 pt
	\tenrm
}


% shorthand
 
\def\larr{\leftarrow}
\def\rarr{\rightarrow}
\def\uarr{\uparrow}
\def\darr{\downarrow}
\def\PA{\partial}
\def\ti{\tilde}
\def\<{\langle}
\def\>{\rangle}
\def\cents{\hbox{\rm\rlap/c}}

% single letters

\def\HI{{\cal H}}
\def\HH{{\Bbb H}}
\def\RR{{\Bbb R}}
\def\CC{{\Bbb C}}
\def\ZZ{{\Bbb Z}}
\def\NN{{\Bbb N}}
\def\MM{{\cal M}}
\def\QQ{{\Bbb Q}}
\def\DD{{\cal D}}
\def\FF{{\cal F}}
\def\BB{{\cal B}}
\def\GG{{\cal G}}
\def\SS{{\bf S}}
\def\TT{{\bf T}}
\def\EE{{\cal E}}
\def\UU{{\cal U}}
\def\II{{\cal I}}
\def\OO{{\cal O}}
\def\Fb{{\bf F}}
\def\ib{{\bf i}}
\def\jb{{\bf j}}
\def\kb{{\bf k}}
\def\rb{{\bf r}}
\def\vb{{\bf v}}
\def\hb{{\bf h}}
% misc math stuff

\def\slim{\mathop{\hbox{\rm s-lim}}}
\def\Ker{\mathop{\rm Ker}}
\def\Ran{\mathop{\rm Ran}}
\def\ad{\mathop{\rm ad}}
\def\Re{\mathop{\rm Re}}
\def\Im{\mathop{\rm Im}}
\def\Log{\mathop{\rm Log}}
\def\Arg{\mathop{\rm Arg}}
\def\tr{\mathop{\rm tr}}
\def\curl{\mathop{\bold curl}}
\def\div{\mathop{\bold div}}
\def\ess{\hbox{\it ess}}
\def\d{\hbox{\it d}}
\def\c{\hbox{\it c}}
\def\pp{\hbox{\it pp}}
\def\jap#1{\langle #1 \rangle}
\def\sph{S^{n\kern -.2ex -\kern -.2ex 1}}
\def\half{$\scriptstyle{{1}\over{2}}$}
\def\DT{{{\partial}\over{\partial t}}}
\def\L{\Delta}
\def\norm#1{\|#1\|}
\def\dint{\int\hskip -5pt \int}
\def\trint{\int\hskip -5pt \int\hskip -5pt \int}
\def\amat4#1#2#3#4#5#6#7#8{
\left[\matrix{
#1\cr
#3\cr
#5\cr
#7\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr#8\cr
}\right]
}

\def\vec4#1#2#3#4{
\left[\matrix{
#1\cr
#2\cr
#3\cr
#4\cr
}\right]
}

\def\amat3#1#2#3#4#5#6{
\left[\matrix{
#1\cr
#3\cr
#5\cr
}\right.\left|\matrix{
#2\cr#4\cr#6\cr
}\right]
}

\def\vec3#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}
 
\def\amat2#1#2#3#4{
\left[\matrix{
#1\cr
#3\cr
}\right.\left|\matrix{
#2\cr#4\cr
}\right]
}
\def\vec2#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}
 
\def\threevec#1#2#3{
\left[\matrix{
#1\cr
#2\cr
#3\cr
}\right]
}

\def\twovec#1#2{
\left[\matrix{
#1\cr
#2\cr
}\right]
}

\def\tr{{\rm tr}}
\def\div{\hbox{\bold div}}
\def\curl{\hbox{\bold curl}}
% misc


%
% 	the stuff after \ifdraftmode only appears if \draftmode has previously 
%	appeared
%
\def\draftmode{\let\dfmd 1}
\def\ifdraftmode#1{\ifx\dfmd 1{#1}\fi}

\def\today{\ifcase\month\or January\or February \or March \or April\or May\or June\or July\or August\or September\or October \or November \or December\fi
\space\number\day, \number\year}

\def\nnarrower{\advance\leftskip by 30pt\advance\rightskip by 30pt}

\def\wwider{\advance\leftskip by -30pt\advance\rightskip by -30pt}

\def\quote#1{{\smallskip\nnarrower\noindent{\it#1}\smallskip}}

\def\hd#1{
\par\penalty-5000
\bigskip\bigskip{\noindent\bold #1}\par\vrule height\bigskipamount width 0pt\penalty10000
}

\def\enum#1{\par\noindent\quad\rlap{#1}\hskip 20pt}

\def\Box{\vbox{\hrule
              \hbox{\vrule height7pt\kern7pt\vrule height7pt}
              \hrule
              }
        }

\def\Picbox{\centerline{
		\vbox{\hrule
                \hbox{\vrule height2.5in\kern5in\vrule height2.5in}
                \hrule
                }
	    }
        }

% 
%	a box of specified height, width and thickness
%

\def\boxhwt#1#2#3{\vbox{\hrule width#2 height#3
                	\hbox{\vrule height#1 width#3 \kern#2\kern-#3\kern-#3 \vrule height#1 width#3}
                	\hrule width#2 height#3
                	      }
        	}
%
%
%	mcomment puts a comment in the margins
%
%
%
%
\def\strutdepth{\dp\strutbox}
%
\newdimen\pagewidth
\newdimen\marginsize

\def\margininsert#1{\strut\vadjust{\kern-\strutdepth
\vtop to \strutdepth{\baselineskip\strutdepth\vss\llap{\marginfont #1}\null}}}
%
\def\marginbox#1{{
\pagewidth=8.5 true in
%	set \marginsize to 1in + \hoffset - .26 true in
	\marginsize=1 true in
	\advance \marginsize by \hoffset
	\advance \marginsize by -.26 true in
\parindent=0pt\raggedright\hsize = \marginsize\vbox{#1}\kern 3pt}}
%
%
\def\mcomment#1{\margininsert{\marginbox{#1}}}

%
%       the following macros read in the files \jobname.eqr 
%       and \jobname .thm which 
%       contain the names of equations and how they are nested 
%       within sections in a format like 
%       \\{name1}\bgnscn\\{name2}\bgnscn\\{name3}\ndscn\ndscn
%       In this example \eqlabelname1 will expand to 1
%                       \eqlabelname2 will expand to 1.1
%                       \eqlabelname3 will expand to 1.1.1
%       This is the maximum nesting supported
%       In the theorem list each \\{name} is preceded by \typetheorem,
%       \typelemma or \typeproposition to indicate what it is
%



\def\bgnsctn{
        \advance\secnest by1
        \cntnumber=0
        \ifnum\secnest=1 
                \advance\seclevelone by1 
                \edef\prenum{\number\seclevelone .}
        \fi
        \ifnum\secnest=2 
                \advance\secleveltwo by1
                \edef\prenum{\number\seclevelone .\number\secleveltwo .}
        \fi
        }
\def\ndsctn{\advance\secnest by-1}

\def\thmtype{} %initialize
\def\typetheorem{\def\thmtype{Theorem}}
\def\typelemma{\def\thmtype{Lemma}}
\def\typeproposition{\def\thmtype{Proposition}}
\def\typecorollary{\def\thmtype{Corollary}}
\def\typehypothesis{\def\thmtype{Hypothesis}}
\def\typeconjecture{\def\thmtype{Conjecture}}
%
% first do the references - define \\ to be a macro which defines \eqlabelname 
% to be a reference number and then evaluate the input string as in Appendix D
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        eqlabel#1\endcsname{\prenum\number\cntnumber}
        }
\newcount\seclevelone \seclevelone=0
\newcount\secleveltwo \secleveltwo=0
\newcount\cntnumber \cntnumber=0
\newcount\secnest \secnest=0
\def\prenum{}
\newread\eqrinfile 
\openin\eqrinfile=\jobname .eqr 
\ifeof\eqrinfile
  \def\eqrinput{\relax}
\else\loop
  \read\eqrinfile to\eqrinput
  \eqrinput
  \ifeof\eqrinfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\eqrinfile

%
% now the same thing for theorems
%
\def\\#1{
        \advance\cntnumber by1
        \expandafter\xdef\csname 
        thmlabel#1\endcsname{\prenum\number\cntnumber}
        \expandafter\xdef\csname 
        typethmlabel#1\endcsname{\thmtype\ \prenum\number\cntnumber}
        }
\seclevelone=0
\secleveltwo=0
\cntnumber=0
\secnest=0
\def\prenum{}
\newread\thminfile 
\openin\thminfile=\jobname .thm
\ifeof\thminfile
  \def\thminput{\relax}
\else\loop
  \read\thminfile to\thminput
  \thminput
  \ifeof\thminfile\let\endfile 1\else\let\endfile 0\fi
  \ifx\endfile 0 \repeat
\fi
\closein\thminfile


        
%
% theorems etc
% These are numbered by section
%

\def\begintheoremlabel#1{
       	\toksdef\ta=0
	\ta={\typetheorem\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Theorem \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endtheoremlabel{\par\medbreak\endgroup}

\def\begintheorem{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begintheoremlabel\temp
}
\def\endtheorem{\endtheoremlabel}

\def\beginlemmalabel#1{
        \toksdef\ta=0
	\ta={\typelemma\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Lemma \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endlemmalabel{\par\medbreak\endgroup}

\def\beginlemma{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginlemmalabel\temp
}
\def\endlemma{\endlemmalabel}



\def\beginpropositionlabel#1{
        \toksdef\ta=0
	\ta={\typeproposition\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Proposition \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endpropositionlabel{\par\medbreak\endgroup}

\def\beginproposition{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginpropositionlabel\temp
}
\def\endproposition{\endpropositionlabel}

\def\begincorollarylabel#1{
        \toksdef\ta=0
	\ta={\typecorollary\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Corollary \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endcorollarylabel{\par\medbreak\endgroup}

\def\begincorollary{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\begincorollarylabel\temp
}
\def\endcorollary{\endcorollarylabel}

\def\beginhypothesislabel#1{
        \toksdef\ta=0
	\ta={\typehypothesis\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Hypothesis \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endhypothesislabel{\par\medbreak\endgroup}

\def\beginhypothesis{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginhypothesislabel\temp
}
\def\endhypothesis{\endhypothesislabel}

\def\beginconjecturelabel#1{
       	\toksdef\ta=0
	\ta={\typeconjecture\\{#1}}
        \immediate\write\thmoutfile{\the\ta}
        \medbreak\par\noindent{\ifdraftmode{\mcomment{#1}}\bf Conjecture \csname thmlabel#1\endcsname}
        \begingroup \it
}
\def\endconjecturelabel{\par\medbreak\endgroup}

\def\beginconjecture{
        \advance\nonamectr by1
        \edef\temp{{noname\the\nonamectr}}
        \expandafter\beginconjecturelabel\temp
}
\def\endconjecture{\endconjecturelabel}





\def\beginproof{\medbreak\par\noindent{\it Proof:\/\ }}
\def\endproof{\thinspace\Box\par\medbreak}

\def\beginproofof#1{\medbreak\par\noindent{\it Proof of #1:\/\ }}
\def\endproofof{\thinspace\Box\par\medbreak}



\def\begindefn{\medbreak\par\noindent{\it Definition:\/\ }}
\def\enddefn{\par\medbreak}

\def\beginexample{\medbreak\par\noindent{\it Example:\/\ }}
\def\endexample{\par\medbreak}

\def\beginexampleset{\beginproblemset}
\def\endexampleset{\endproblemset}


\def\beginremark{\medbreak\par\noindent{\it Remark:\/\ }}
\def\endremark{\par\medbreak}

\def\beginremarkno#1{\medbreak\par\noindent{\it Remark #1:\/\ }}
\def\endremarkno{\par\medbreak}



%-------------------------------------------------------
%	no longer needed
%
%       \appendtxt appends the text in #2 to the token list 
%       contained in the token variable #1
%
\def\appendtxt#1#2{ 
        \toksdef\ta=0
        \ta=\expandafter{\the#1#2}
        \global#1=\expandafter{\the\ta}
        }
%----------------------------------------------------------

%
%
%	open files for writing
%
%
\newwrite\eqroutfile 
\immediate\openout\eqroutfile=\jobname .eqr 
\newwrite\thmoutfile 
\immediate\openout\thmoutfile=\jobname .thm


%
%       \be{name} and \ee begin and end a numbered displayed equation 
%       the tokens in the name are added to the token list in \eqrtoks
%       if \eqlabelname has been defined uses this as a number
%       \lastdisplayline{name}{...} gives a referenced number  to the last 
%       line in a displaylines series
%
\def\be#1{
        \def\temp{#1}
	\toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}$$
	}
\def\ee{
        \eqno{(\csname eqlabel\temp\endcsname)
	\ifdraftmode{\rlap{\ {\marginfont\temp}}}}$$
        }
\def\lastdisplayline#1#2{
        \hfill#2\hfill{\rm\llap{(\csname eqlabel#1\endcsname)}
	\ifdraftmode{\rlap{\ {\marginfont#1}}}}\cr
        \toksdef\ta=0
	\ta={\\{#1}}
        \immediate\write\eqroutfile{\the\ta}
        }

%
%       \beginsection begins a new section
%       writes \bgnsctn to token list in \eqrtoks
%       \endsection ends a section
%       writes \ndsctn to token list in \eqrtoks
%
\def\beginsection{
        \advance\secnumber by1
        \probctr=0
	\toksdef\ta=0
	\ta={\bgnsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }
\def\endsection{
        \toksdef\ta=0
	\ta={\ndsctn}
        \immediate\write\eqroutfile{\the\ta}
        \immediate\write\thmoutfile{\the\ta}
        }

%
%       \rf{name} inserts (<number>) where <number> is the equation number
%       referred to by "name"
%
\def\rf#1{(\csname eqlabel#1\endcsname )}

%
%       \thmrf is the analogous thing for theorems
%
%\def\thmrf#1{\hbox{\csname typethmlabel#1\endcsname}}
\def\thmrf#1{\csname typethmlabel#1\endcsname}







\def\chead#1{\medbreak\centerline{#1}\medskip}

\def\bea#1{$$\eqalign\begingroup}
\def\eea{\endgroup $$}
\def\beann{$$\eqalign\begingroup}
\def\eeann{\endgroup $$}


%
%       some lecture note macros
%
\def\beginlecture{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber}
        \medskip
}
\def\endlecture{\endsection\vfill\eject}
%
%
%
\def\beginlecturetitle#1{
        \beginsection 
        \probctr=0
        \par\noindent{\bf Lecture \number\secnumber : #1}
        \medskip
}
\def\endlecturetitle{\endsection\vfill\eject}
%
%
%
\def\readsec#1{\medskip{\sl Reading:} Section #1}
\def\readsecs#1{\medskip{\sl Reading:} Sections #1}
\def\hmk#1#2{\medskip{\sl Problems (due #1): }#2}
%
%       sec macro
%
\def\beginsec#1{
	\bigskip
        \beginsection 
        \par\noindent\centerline{\bf \number\secnumber . #1}
        \medskip
}
\def\endsec{\endsection\par}

\def\beginproblem{
        \advance\probctr by1
        \medbreak\par\noindent
        {\it Problem \number\secnumber .\number\probctr:\/}
}
\def\endproblem{\par\medbreak}

\def\ans{{\medskip\bold Answer: }}

\def\beginsolution{
        \medbreak\par\noindent
        {\it Solution \number\secnumber .\number\probctr:\/}
}
\def\endsolution{\par\medbreak}

\def\beginproblemset{\bigskip\hrule\bigskip\advance\leftskip by 30pt
\advance\rightskip by 30pt\smallfont}
\def\endproblemset{\bigskip\hrule\bigskip\advance\leftskip by -30pt
\advance\rightskip by -30pt\normalfont}
\def\bsp{\beginproblemset\beginproblem}
\def\esp{\endproblem\endproblemset}


%
%	some research note macros
%

\def\beginnote#1{
	%\magnification 1100
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt
        \beginsection 
        \probctr=0
        \par\noindent\centerline{\bf #1}
	\centerline{filename: {\tt\jobname .tex}}
	\centerline{\today}
        \medskip
}
\def\endnote{\endsection\vskip 20pt}


\def\notefontsize{
	\hsize = 5.9 true in
	\hoffset = 0.45 true in
	\baselineskip = 18pt}

%
%       These go at the beginning  of input
%
\global\newtoks\eqrtoks
\global\newtoks\thmtoks
\global\newcount\secnumber
\global\newcount\nonamectr
\global\newcount\probctr



\def\rixend{\closeout\eqroutfile \closeout\thmoutfile \vfill\eject\end}

\message{*** reference macros need to run twice to get references right ***}


==> statement.tex <==
\hd{Abstract}

We give a new proof of a version of Klein's theorem on the
existence of absolutely continuous spectrum for the Anderson
model on the Bethe Lattice at weak disorder.

\hd{Model and Statement of Main Results}

It is widely believed that the Anderson model [An] should exhibit absolutely continuous
spectrum at weak disorder in dimensions three and higher. But it is only 
for the Bethe lattice $\Bbb{B}$, or Cayley tree, that this has been established.
The first proof was given by Klein [K1, K2], and his remained the only result of this
kind until the recent work of Aizenman, Sims and Warzel [ASW]. These authors
proved a stability result for absolutely continuous spectrum for the Anderson
model on $\Bbb{B}$ that implies the existence of an absolutely continuous component in the spectrum
for perturbations of the Anderson model on $\Bbb{B}$, also in the presence of a periodic background
potential. 
For the related problem of proving absolutely continuous spectrum for slowly decaying
potentials there has been recent progress ([D], [KLS], [SS]). It is interesting to note that for the Bethe lattice,
localization for large disorder has not yet been established at the band edge,
but only for strictly larger energies (see [Ai], [AM]). For more information about this
model, and further references we recommend the discussion in [ASW].

In this paper we give a new proof of a variant of Klein's theorem, \thmrf{Klein}
below. Our proof is quite different from either of the
two previous approaches. It is based on [FHS] where we proved existence of absolutely continuous spectrum for
a class of deterministic potentials whose radial behaviour was restricted
only by an $\ell^\infty$ bound. That proof was based on the contracting properties
of the map $\phi$, defined below, that arises in the recurrence relation for the Green's function,
thought of as a map between hyperbolic spaces. Our \thmrf{mu3bdd} is a version of this,
adapted to the probabilistic setting. Klein is able to handle some random potentials that
we cannot, since we require that the single site distribution has a finite fourth moment. 
On the other hand, our \thmrf{Zdecay} quantifies how the finiteness of higher moments of  
the single site distribution leads to more decay in the probability
distribution of the Green's function.

The Bethe Lattice, $\Bbb{B}$, or Cayley tree of degree $k$ is 
the infinite connected graph with no closed loops where each vertex 
has $k$ nearest neighbours. In this paper, we set $k=3$. We
believe a similar proof should work for all $k$. But a proof along
our lines for larger $k$ would involve, at the least, greater notational complexity.

The Anderson model on 
$\Bbb{B}$ is given by the random Hamiltonian 
$$
H = \L + q
$$  
on the Hilbert space 
$$
{\cal H} = \ell^2(\Bbb{B}) = \left\{ \, \varphi : \Bbb{B} \to  \Bbb{C}  \, : \, \sum_{x \in \Bbb{B}} | \varphi(x) |^2 < \infty \, \right\} \, ,
$$
where 
$q$ denotes a random potential, such that for each $x \in \Bbb{B}$, $q(x)$ is an independently
distributed real 
random variable with probability distribution $\nu$,
and
$\L$ is the Laplacian defined by
$$
(\L \varphi)(x) = \sum_{y : {\rm d}(x,y) = 1 } \varphi(y) \,. 
$$ 
Here ${\rm d}(x,y)$ denotes the distance in the graph, that is, the number
of edges in the shortest path joining $x$ and $y$.
The spectrum of the free Laplacian is  
$\sigma(\Delta) = [ - 2 \sqrt{2} , 2 \sqrt{2} ]$. The main theorem
which we will prove is the following.

\begintheoremlabel{Klein}
For any $E$, with $0 < E <2 \sqrt{2}$, there exist $\delta_1 > 0$ and $\delta_2 > 0$, 
such that for all $\nu$ with 
$$\eqalign{
%\int_{|q|\ge\delta_1} d\nu(q) &\le \delta_2\,,\cr
\int_{|q|\ge\delta_1} (1+|q|^4) \,d\nu(q) &\le \delta_2\,,\cr
}$$ 
the spectrum of $H$ is purely
absolutely continuous in $[-E,E]$ with probability one, i.e., we have almost 
surely
$$
\Sigma_{\rm ac} \cap [-E,E] = [-E, E] \ , \ \ \Sigma_{\rm pp} \cap [-E,E] = \emptyset \ , \ \ 
\Sigma_{\rm sc} \cap [ -E, E] = \emptyset \; . 
$$
\endtheoremlabel
\noindent 
As was shown in [K], \thmrf{Klein} follows from the following fact.
Let $R(E,\epsilon)$ be the strip in the complex plane defined by
$$ 
R(E,\epsilon) = \{ z \in \HH  \, : \, 
{\rm Re} z \in [-E,E], \,  0 < {\rm Im} z \leq \epsilon \}\,.
$$ 
\begintheoremlabel{Klein2}
Let $x \in \Bbb{B}$. Under the hypotheses of \thmrf{Klein},
$$
\sup_{\lambda \in R(E,\epsilon) } 
{\Bbb E}  \left( \left| \langle  x | (H - \lambda)^{-1} | x \rangle \right|^2 \right) 
< \infty \; 
$$ 
for some $\epsilon > 0$.
\endtheoremlabel

Here is a brief outline of the paper. Our main technical result is the contraction
estimate in \thmrf{mu3bdd}. This and the companion result \thmrf{mu3qbdd}
are used in \thmrf{Zdecay} to prove that the probability distribution on the 
hyperbolic plane for $Z^{(x|y)}(\lambda)$, defined below, decays at infinity.
This decay then implies the decay of the Green's function required in 
\thmrf{Klein2}.

Let $\HH = \{z\in\CC : \Im(z) > 0\}$ denote the complex upper half plane.
For convenience we fix an arbitrary site in $\Bbb{B}$ to be the origin and denote it by 0.
Given two nearest neighbour sites $x,y \in \Bbb{B}$, we will denote by $\Bbb{B}^{(x|y)}$ the graph 
obtained by removing from $\Bbb{B}$ the branch emanating from $x$ that passes through $y$.
We will write $H^{(x|y)}$ for $H$ when restricted to $\Bbb{B}^{(x|y)}$ and set
$$
G^{(x|y)}(\lambda) = \langle x | ( H^{(x|y)}  - \lambda )^{-1} | x \rangle \; .
$$
We will use the following recursion relations. For a proof see [K] or
[FHS].

\beginproposition
For any $\lambda \in \Bbb{H}$,
\be{rel:Gg}
G(0,0,\lambda)
=\langle 0 | (H - \lambda)^{-1} | 0 \rangle 
= - \left( \sum_{x:\dist(x,0)=1} G^{(x|0)}(\lambda) + \lambda - q(0) \right)^{-1} \, ,
%= {{-1}\over{\sum_{x:\langle x 0 \rangle} G^{(x|0)} + \lambda - q(0)}}
\ee
and for any two nearest neighbour sites $x,y \in \Bbb{B}$
\be{rel:gg}
G^{(x|y)}(\lambda) 
= - \left( \sum_{x':\,{\rm d}(x,x')=1,x'\neq y}  G^{(x'|x)}(\lambda) 
+ \lambda - q(x) \right)^{-1} \, .
\ee
\endproposition

It will turn out to be convenient to study 
the sum of two Green's functions, i.e., for two nearest neighbour sites
$x,y \in \Bbb{B}$ we set
\be{rel:Zg}
Z^{(x|y)}(\lambda) = \sum_{x':\,{\rm d}(x,x')=1,x'\neq y} G^{(x'|x)}(\lambda) \; .
\ee
Using the recursion relation for $G^{(x|y)}(\lambda)$ we obtain the following recursion
relation
$$
Z^{(x|y)}(\lambda) 
= -  \sum_{x':\,{\rm d}(x,x')=1,x'\neq y}
\left( Z^{(x'|x)}(\lambda) + \lambda - q(x')  \right)^{-1} \; .
$$
This leads to the investigation of the 
transformation $\phi:\HH\times\HH\times \RR \times \RR \times \HH \to \HH$
defined by
\be{phi}
\phi(z_1,z_2,q_1,q_2,\lambda) 
= {{-1}\over{z_1+\lambda-q_1}} 
+ {{-1}\over{z_2+\lambda-q_2}} \; .
\ee
If ${\rm Im} \lambda > 0$,
the transformation $z\mapsto\phi(z,z,0,0,\lambda)$
has a unique  fixed point, $z_\lambda$,  in the upper half plane, i.e,
with ${\rm Im} z_\lambda > 0$.
Explicitly,
$$
z_\lambda = -\lambda/2 + \sqrt{(\lambda/2)^2-2} \; ,
$$
where we will always make the 
choice ${\rm Im} \sqrt{ \, \cdot \, } \geq 0$ (and 
$\sqrt{ a} > 0$ for $a>0$). This fixed point as a function
of $\lambda \in \HH$ extends continuously onto the real axis. 
This extension yields for 
$\Im(\lambda) = 0$ and $|\lambda|< 2 \sqrt{2}$ the fixed point
$$
z_\lambda = -\lambda/2 + i \sqrt{2 - (\lambda/2)^2} \;,
$$
lying on an arc of the circle $|z|=\sqrt{2}$. When $\Im(\lambda) = 0$
and $|\lambda|\le E < 2 \sqrt{2}$, the arc is strictly
contained in the upper half plane. Thus when $\lambda$ lies in the strip
$R(E,\epsilon)$
with
$0<E<2\sqrt{2}$ and $\epsilon$ sufficiently small, $\Im(z_\lambda)$
is bounded below and $|z_\lambda|$ is bounded above by a positive constant.

We will use the weight function $\cd(z)$ defined by
\be{cddefn}
\cd(z) = 2\Im(z_\lambda)(\cosh({\rm dist}_\HH(z,z_\lambda))-1) = {{|z-z_\lambda|^2}\over{\Im(z)}} \; .
\ee
Up to 
constants,
$\cd(z)$ is the hyperbolic cosine of the 
hyperbolic distance from $z$ to $z_\lambda$, provided $\lambda\in R(E,\epsilon)$ 
with $0<E<2\sqrt{2}$ and $\epsilon$ sufficiently small. This notation
suppresses the $\lambda$ dependence.

To prove \thmrf{Klein2}, we will study the following function
\be{mu3pdefn}
\mu_{3,p}(z_1,z_2,z_3,q_1,q_2,q_3,q_4, \lambda) =
\sum_{\sigma} {{{\rm cd}^p(\phi(z_{\sigma_1}, \phi(z_{\sigma_2}, z_{\sigma_3},
q_{\sigma_2},q_{\sigma_3}, \lambda), q_{\sigma_1},q_4,\lambda))}\over{
{\rm cd}^p(z_1) + {\rm cd}^p(z_2) + {\rm cd}^p(z_3) }} \; ,
\ee
where $\sigma$ runs over the cyclic permutations of $(1,2,3)$, i.e.,
$(\sigma_1,\sigma_2,\sigma_3) \in \{ (1,2,3), (2,3,1), (3,1,2) \}$. Note 
that $\mu_{3,p}$ is well defined as long as $(z_1,z_2,z_3) \neq (z_\lambda, z_\lambda, z_\lambda)$.
The  proof of \thmrf{Klein}  is based on the following bounds, which will
be proved in the next section. For small $|q_i|$ we have

\beginlemmalabel{mu3bdd}
For any $E$, $0 < E  < 2 \sqrt 2$ and any $p>1$, there exist positive constants
$ \epsilon$ , $\delta$, $\epsilon_0$
and a compact  set $K \subset \HH^3$ such that 
\be{mu3pest1}\eqalign{
\mu_{3,p} \big|_{K^c \times [-\delta, \delta]^4 \times R(E,\epsilon_0)} &\le 1 - \epsilon \,. \cr
}\ee
Here $K^c$ denotes the complement $\HH^3\backslash K$.
\endlemmalabel
\noindent 
This theorem also holds for $p=1$, but the proof is more involved.
We will also need the following bounds, that hold for all $|q_i|$.
\beginlemmalabel{mu3qbdd}
For any $E$, $0 < E  < 2 \sqrt 2$ and any $p\ge 1$, there exist positive constants
$\epsilon_0$, $C$
and a compact  set $K \subset \HH^3$ such that 
\be{mu3pest2}\eqalign{
\mu_{3,p} \big|_{K^c \times \RR^4 \times R(E,\epsilon_0)} &\le C\left(1+\sum_{i=1}^4|q_i|^{2p}\right)\,. \cr
}\ee
Similarly, if we define 
$$\eqalign{
\mu'_{3,p}(z_1,z_2,z_3,q,\lambda) &= {{\cd(-(z_1+z_2+z_3+\lambda-q)^{-1})^p}\over{\cd(z_1)^p+\cd(z_2)^p+\cd(z_3)^p}}\,,\cr
\mu'_{1,p}(z,q,\lambda) &= {{\cd(-(z+\lambda-q)^{-1})^p}\over{\cd(z)^p}}\,,\cr
}$$
then
$$\eqalign{
\mu'_{3,p} \big|_{K^c \times \RR^4 \times R(E,\epsilon_0)} &\le C\left(1+|q|^{2p}\right)\,, \cr
\mu'_{1,p} \big|_{K^c \times \RR^4 \times R(E,\epsilon_0)} &\le C\left(1+|q|^{2p}\right)\,. \cr
}$$
\endlemmalabel

Let $\rho$ be the probability distribution for
$Z^{(0|x)}(\lambda)$ on the hyperbolic plane given by
$$
\rho(A) = {\rm Prob}( Z^{(0|x)}(\lambda) \in A ) \,  .
$$
Although it is suppressed in the notation, $\rho$ depends on $\lambda$, 
and for $\Im(\lambda)>0$ the support of $\rho$ is bounded. This follows, for example 
from the fact that it is contained in the range of $\phi$. 
Given \thmrf{mu3bdd} and \thmrf{mu3qbdd}, we can prove that the decay of $\rho$
at infinity is preserved as $\Im(\lambda)$ becomes small,
provided $\nu$ has enough
finite moments and is concentrated near $0$. 
\begintheoremlabel{Zdecay} Let $x$ be a nearest neighbour of $0$.
For any $E$, $0<E<2\sqrt{2}$ and $p>1$, there exist $\delta_1 > 0$, $\delta_2 > 0$ and $\epsilon>0$, 
such that for all $\nu$ satisfying
$$\eqalign{
%\int_{|q|\ge\delta_1} d\nu(q) &\le \delta_2\,,\cr
\int_{|q|\ge\delta_1} (1+|q|^{2p}) d\nu(q) &\le \delta_2\,,\cr
}$$ 
we have
$$
\sup_{\lambda \in R(E,\epsilon)} \Bbb{E} \left(  {\rm cd}^p(Z^{(0|x)}(\lambda)) \right) 
 < \infty \; .
$$
\endtheoremlabel
\beginproof
Let $\delta_1$ be the $\delta$ given by \thmrf{mu3bdd}, and choose $\epsilon_0$ and
$K$ that work in both \thmrf{mu3bdd} and \thmrf{mu3qbdd}.
For $(z_1,z_2,z_3)\in K^c$, we estimate
$$\displaylines{\quad
\int_{\RR^4} \mu_{3,p}(z_1,z_2,z_3,q_1,\ldots,q_4,\lambda)\; d\nu(q_1)\ldots d\nu(q_4)
\hfill\cr\hfill\eqalign{
&\le (1-\epsilon)\int_{[-\delta_1,\delta_1]^4}d\nu(q_1)\ldots d\nu(q_4)
+C\int_{\RR^4\backslash[-\delta_1,\delta_1]^4}(1+\sum_{i=1}^4|q_i|^{2p})\,d\nu(q_1)\ldots d\nu(q_4)\cr
&\le (1-\epsilon) + 
C\left(1+4M_{2p} - \left(\int_{[-\delta_1,\delta_1]}d\nu(q)\right)^4
-4\left(\int_{[-\delta_1,\delta_1]}d\nu(q)\right)^3\int_{[-\delta_1,\delta_1]}|q|^{2p}d\nu(q)\right)\cr
&\le (1-\epsilon) + C\big(1+4M_{2p} -(1-\delta_2)^4 - 4(1-\delta_2)^3(M_{2p}-\delta_2)\big)\cr
&\le 1-\epsilon/2\cr
}\quad}$$
provided $\delta_2$ is sufficiently small. Here $M_{2p}$ denotes the moment
$\int |q|^{2p}\,d\nu(q)$.

The recursion relation for $Z^{(0|x)}(\lambda)$  implies that for any
continuous function $w(z)$
$$
\int_\HH w(z) d\rho(z) = \int_{\HH\times\HH\times\RR\times\RR} w(\phi(z_1,z_2,q_1,q_2,\lambda))\,d\rho(z_1)d\rho(z_2)\,d\nu(q_1)d\nu(q_2).
$$
Using this relation (twice) and the estimate above, we obtain
for $\lambda \in R(E,\epsilon_0)$,
$$\displaylines{\quad
\Bbb{E}\left({\rm cd}^p(Z^{(0|x)})(\lambda) \right) 
\hfill\cr\hfill \eqalign{
& = \int {\rm cd}^p(z)\, d \rho(z) 
\cr
& = \int {\rm cd}^p( \phi(z_1,z_2,q_1,q_2,\lambda)\,
d\rho(z_1) d\rho(z_2)\, d\nu(q_1) d\nu(q_2) 
\cr
& = \int {\rm cd}^p( \phi( z_1 ,\phi(z_2,z_3,q_2,q_3,\lambda),q_1,q_4,\lambda) )\,
d\rho(z_1) \ldots  d\rho(z_3 )\, d\nu(q_1) \ldots  d\nu(q_4) 
\cr
& = \int {1\over3} \sum_\sigma {\rm cd}^p\big(\phi(z_{\sigma_1}, 
\phi(z_{\sigma_2}, z_{\sigma_3}, q_{\sigma_2},q_{\sigma_3},\lambda) q_{\sigma_1},
q_{\sigma_4}, \lambda))\big)\, d\rho(z_1) \ldots  d\rho(z_3)\, d\nu(q_1) \ldots 
d\nu(q_4) 
\cr
& = {1\over3} \int_{K^c}\left(\int_{\Bbb{R}^4} \mu_{3,p}(z_1,z_2,z_3,q_1,\ldots ,q_4,\lambda)\,d\nu(q_1) \ldots 
d\nu(q_4)\right) 
\cr 
& \quad \times \big(
{\rm cd}^p(z_1) + {\rm cd}^p(z_2) + {\rm cd}^p(z_3) \big)\,d\rho(z_1) \ldots  d\rho(z_3)  + C 
\cr
& \le ( 1 - \epsilon/2) \int {\rm cd}^p(z)\, d \rho(z) + C   \, , 
}\quad}
$$
where $C$ is some finite constant, only depending on the choice of $K$.
This implies that for all $\lambda \in R(E,\epsilon_0)$,
$$
\Bbb{E} \left( {\rm cd}^p( Z^{(0|x)} )  \right) \leq {2C \over{\epsilon} } \; .
$$
\endproof

Now we show how this theorem for $p=2$ implies \thmrf{Klein2}. We must transfer
our decay estimate for the distribution $\rho$ for $Z^{(0|x)}(\lambda)$ to the distributions
$\rho_g$ for $G^{(0|x)}(\lambda)$ and finally to $\rho_G$ for $G(0,0,\lambda)$, where these
probability distributions are defined by
by
$$
\eqalign{
\rho_G(A) &= {\rm Prob} \{ G(0,0,\lambda) \in A \}\,, \cr
\rho_g(A) &= {\rm Prob} \{ G^{(0|x)}(\lambda) \in A \}  \,.
}$$
\beginproofof{\thmrf{Klein2}}
We will
use the following inequality:
\be{ineq:abs}
|z| \leq 4 {{|z-w|^2}\over{{\rm Im}z}} + 2 |w| \; .
\ee
The inequality
clearly holds for $|z| \leq 2 |w|$. In the complementary case, we have   
$|z| > 2 |w|$ and thus
$|z-w| \geq ||z|-|w|| \geq |w|$, implying
$$
|z|{\rm Im}z \leq |z|^2 \leq 2 |z-w|^2 + 2 |w|^2 \leq 4 |z - w|^2 \; 
$$
and further $|z| \leq 4 |z-w|^2/{\rm Im}z$.  This proves \rf{ineq:abs}.

Using \rf{ineq:abs} with $w=z_\lambda$ yields that for $\lambda\in R(E,\epsilon)$
$$
|z| \le 4 \cd(z) + C\,,
$$
where $C$ depends only on $E$ and $\epsilon$.
To transfer the estimate on $\rho_g$ to one on
$\rho_G$ we use the relation \rf{rel:Gg} and the estimate
on $\mu'_{3,2}$ given by \thmrf{mu3qbdd}. Let $R$ denote $R(E,\epsilon)$. Then
$$\displaylines{\quad
{\rm sup}_{\lambda \in R} \Bbb{E} \left( \left| \left\langle
0 | ( H-\lambda )^{-1}  | 0 \right\rangle \right|^2 \right)
\hfill\cr\hfill
\eqalign{
&= {\rm sup}_{\lambda \in R} \int |z|^2 \,d\rho_G(z) \cr
&\leq  32 \, {\rm sup}_{\lambda \in R} \int \cd^2(z)  \,d\rho_G(z) + C \cr
&= 32 \, {\rm sup}_{\lambda \in R} \int \cd^2(-1/(z_1+z_2+z_3+\lambda - q ))\,
d\rho_g(z_1) d\rho_g(z_2) d\rho_g(z_3) \,d\nu(q) + C \cr
&\le 32 \, {\rm sup}_{\lambda \in R} \int_{K^c\times\RR} \mu'_{3,2}(z_1,z_2,z_3,q,\lambda)\cr
&\quad\quad \times(\cd^2(z_1)+\cd^2(z_2)+\cd^2(z_3))\,
d\rho_g(z_1) d\rho_g(z_2) \,d\rho_g(z_3) \,d\nu(q) + C \cr
&\le C \int_{\HH\times\RR}(1+|q|^4)\cd^2(z) \,d\rho_g(z)\,d\nu(q) + C\cr
&\le C\int\cd^2(z) \,d\rho_g(z) + C\,.\cr
}\quad}$$
A completely analogous argument, using the relations \rf{rel:gg} and \rf{rel:Zg}
and the estimate of $\mu'_{1,p}$ in \thmrf{mu3qbdd} yields
$$
\int\cd^2(z) \,d\rho_g(z) \le C \int\cd^2(z) \,d\rho(z) + C
$$
and completes the proof.
\endproof

